The Devil is in the GAN: Backdoor Attacks and Defenses in Deep Generative Models

Deep Generative Models (DGMs) are a popular class of deep learning models which find widespread use because of their ability to synthesize data from complex, high-dimensional manifolds. However, even with their increasing industrial adoption, they haven't been subject to rigorous security and privacy analysis. In this work we examine one such aspect, namely backdoor attacks on DGMs which can significantly limit the applicability of pre-trained models within a model supply chain and at the very least cause massive reputation damage for companies outsourcing DGMs form third parties. While similar attacks scenarios have been studied in the context of classical prediction models, their manifestation in DGMs hasn't received the same attention. To this end we propose novel training-time attacks which result in corrupted DGMs that synthesize regular data under normal operations and designated target outputs for inputs sampled from a trigger distribution. These attacks are based on an adversarial loss function that combines the dual objectives of attack stealth and fidelity. We systematically analyze these attacks, and show their effectiveness for a variety of approaches like Generative Adversarial Networks (GANs) and Variational Autoencoders (VAEs), as well as different data domains including images and audio. Our experiments show that - even for large-scale industry-grade DGMs (like StyleGAN) - our attacks can be mounted with only modest computational effort. We also motivate suitable defenses based on static/dynamic model and output inspections, demonstrate their usefulness, and prescribe a practical and comprehensive defense strategy that paves the way for safe usage of DGMs.

==> custom_commands.tex <==
\usepackage{todonotes}

%
% e.g: \newacronym{gm}{GM}{Generative Models}
%
%
\usepackage[acronym]{glossaries}

%Allows the creation of tables combining rows and columns
%https://www.overleaf.com/learn/latex/Tables#Combining_rows_and_columns
\usepackage{multirow}

%
% e.g: \missingtext{Institution Name 1}
%
% turns the text red and adds a corresponding todo in the list. 
\newcommand{\missingtext}[1]{%
{\textbf{\color{red}{#1}}}\addcontentsline{tdo}{todo}{\textbf{Missing Text: }#1}%
}


%
% e.g: \comment[AuthorName]{Comment}
%
% adds an in-line todo in light green

\usepackage{ifthen}

\newcommand{\comment}[2][]{%
\ifthenelse { \equal {#1} {} }%  %if no author was given for the comment
{\todo[color={green!40}]{\textbf{Comment:~}#2}}   % then
{\todo[color={green!40}]{\textbf{Comment (#1):~}#2}}   % else (not blank) 
}



%
% e.g: \assigntodo[Assignee]{Task}
%
% adds an in-line todo in light green

\newcommand{\assigntodo}[2][]{%
\ifthenelse { \equal {#1} {} }%  %if no author was given for the comment
{\todo[color={red!50}]{\textbf{TODO:~}#2}}   % then
{\todo[color={red!50}]{\textbf{TODO [@#1]:~}#2}}   % else (not blank) 
}


